A Multi-Layered Approach for Measuring the Simulation-to-Reality Gap of Radar Perception for Autonomous Driving

With the increasing safety validation requirements for the release of a self-driving car, alternative approaches, such as simulation-based testing, are emerging in addition to conventional real-world testing. In order to rely on virtual tests the employed sensor models have to be validated. For this reason, it is necessary to quantify the discrepancy between simulation and reality in order to determine whether a certain fidelity is sufficient for a desired intended use. There exists no sound method to measure this simulation-to-reality gap of radar perception for autonomous driving. We address this problem by introducing a multi-layered evaluation approach, which consists of a combination of an explicit and an implicit sensor model evaluation. The former directly evaluates the realism of the synthetically generated sensor data, while the latter refers to an evaluation of a downstream target application. In order to demonstrate the method, we evaluated the fidelity of three typical radar model types (ideal, data-driven, ray tracing-based) and their applicability for virtually testing radar-based multi-object tracking. We have shown the effectiveness of the proposed approach in terms of providing an in-depth sensor model assessment that renders existing disparities visible and enables a realistic estimation of the overall model fidelity across different scenarios.

==> sections/02_related_work.tex <==
\section{Related Work}
\label{sec: related work}


state of the art of simulation evaluation and credibility? -> how to evaluate a simulation model
- standards
	- NASA
	- IEEE UMP? check correct name
- projects? pegasus etc.
	- see SL425 report!
- research (paper)
	- which interface for evaluation?
	
-> existing testing methods -> not detailed enough for sensor simulations?
similar to NASA credibility assessment levels -> but here more hands on and directly applicable to sensor simulation
- e.g. NASA 4 levels for validation 
-> level 4 (highest) -> all outputs of Simulation agree with Real World System (does it mean every interface) in full range of operation -> and how to measure metrics etc 
-> level 3 - all key outputs ... in representative environment -> what are key outputs, metrics and agree how much? etc. 
	

\subsection{Sensor Model Types}

% existing sensor model defintions:
- ideal or ground truth model
- phenomenological model
- stochastic, data-driven model
- physical model

white, grey, black box model

2020-schlager:
- low-fidelity model
- medium-fidelity model
- high-fidelity model




\subsection{Quantify Simulation-to-Reality Gap}
% testing sensor models
- camera model testing -> simulation to reality gap based on object detection results \cite{reway_test_2020}

- camera -> 2020 hoeber -> also evaluation in frequency domain

hartstern2020 -> also V-model but for sensor setup -> is a good example for sensor model usecase

metrics? % TODO: cite deepeval? -> or double citation at ray casting model?


%TODO: Check out testing methods from statistics - Kolmogorov-Smirnov-Test, Agnostic tests etc. → when to use?

% TODO: Check out TRL on confluence in confluence Technology+Readiness+Level+(TRL)+Definitions


metrics? % TODO: cite deepeval? -> or double citation at ray casting model?




- what are relevant existing approaches and what is missing?
TODO: check for relevant works -> does anyone did this or something similar before? -> add them to .tex -> depending on size create extra section
regarding problem 1:
• 2019 rosenberger benchmark
◇ tackles this problem? explicit and implicit -> but lacks to determine what is enough and not detailed? TOCHECK
• reway test 2020
◇ camera model testing -> simulation to reality gap based on object detection results

regarding problem 2:
• 2019 rosenberger towards:
◇ proposed method concept for validation
◇ -> but no results? and does they show exactly what is sufficient? TOCHECK
• 2020 schlager sensor models
◇ proposed taxonomy for sensor models
◇ mapping sensor model fidelity types to V-Model
◇ -> but definition based on modeling approach - e.g. rendering -> high fidelity -which is not generally valid (describes IMHO more the potential)





